Dynamic Matrix Inverse: Improved Algorithms and Matching Conditional Lower Bounds

The dynamic matrix inverse problem is to maintain the inverse of a matrix undergoing element and column updates. It is the main subroutine behind the best algorithms for many dynamic problems whose complexity is not yet well-understood, such as maintaining the largest eigenvalue, rank and determinant of a matrix and maintaining reachability, distances, maximum matching size, and $k$-paths/cycles in a graph. Understanding the complexity of dynamic matrix inverse is a key to understand these problems. In this paper, we present (i) improved algorithms for dynamic matrix inverse and their extensions to some incremental/look-ahead variants, and (ii) variants of the Online Matrix-Vector conjecture [Henzinger et al. STOC'15] that, if true, imply that these algorithms are tight. Our algorithms automatically lead to faster dynamic algorithms for the aforementioned problems, some of which are also tight under our conjectures, e.g. reachability and maximum matching size (closing the gaps for these two problems was in fact asked by Abboud and V. Williams [FOCS'14]). Prior best bounds for most of these problems date back to more than a decade ago [Sankowski FOCS'04, COCOON'05, SODA'07; Kavitha FSTTCS'08; Mucha and Sankowski Algorithmica'10; Bosek et al. FOCS'14]. Our improvements stem mostly from the ability to use fast matrix multiplication ``one more time'', to maintain a certain transformation matrix which could be maintained only combinatorially previously (i.e. without fast matrix multiplication). Oddly, unlike other dynamic problems where this approach, once successful, could be repeated several times (``bootstrapping''), our conjectures imply that this is not the case for dynamic matrix inverse and some related problems. However, when a small additional ``look-ahead'' information is provided we can perform such repetition to drive the bounds down further.

==> all_reductions_table.tex <==

\begin{figure}
\center
% Preview source code for paragraph 0
\small
% Preview source code for paragraph 0

\begin{tabular}{ll|ll}
\hline 
\multicolumn{2}{c|}{inverse} & \multicolumn{2}{c}{matrix product}\tabularnewline
\hline 
matrix product  & \Cref{thm:matrixProductReduction}  & largest singular/eigen-value  & \Cref{thm:eigenValueVectorReduction} \tabularnewline
determinant  & \Cref{thm:inverseDeterminantEquivalence}  & subgraph triangle detection  & \Cref{thm:subgraphTriangleDetectionReduction} \tabularnewline
adjoint  & \Cref{cor:inverseAdjointEquivalence}  & triangle detection  & \Cref{thm:nodeUpdateTriangleDetectionReduction} \tabularnewline
linear system  & \Cref{thm:linearSystemReduction}  & k-path  & \Cref{thm:kPathReduction} \tabularnewline
pseudo inverse  & \Cref{thm:pseudoInverseReduction}  &  & \tabularnewline
polynomial inverse  & \Cref{cor:polyElementUpdate}  &  & \tabularnewline
DAG path counting  & \Cref{thm:DAGcounting}  &  & \tabularnewline
 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c}{}\tabularnewline
\hline 
\multicolumn{2}{c|}{determinant} & \multicolumn{2}{c}{polynomial inverse}\tabularnewline
\hline 
rank  & \Cref{thm:rankReduction}  & adjoint (division free)  & \Cref{cor:ringAdjointDeterminant} \tabularnewline
perfect matching  & \Cref{thm:perfectMatchingReduction}  & determinant (division free)  & \Cref{cor:ringAdjointDeterminant} \tabularnewline
cycle detection  & \Cref{thm:cycleDetectionReduction}  & k-cycle  & \Cref{thm:kCycleReduction} \tabularnewline
 & \multicolumn{1}{c|}{} & st-distance  & \multicolumn{1}{c}{\Cref{thm:shortestDistanceReduction} }\tabularnewline
 & \multicolumn{1}{l}{} &  & \tabularnewline
\hline 
\multicolumn{2}{c|}{linear system} & \multicolumn{2}{c}{adjoint}\tabularnewline
\hline 
interpolation polynomial  & \Cref{thm:interpolationPolynomial}  & transitive closure  & \Cref{thm:transitiveClosureReduction} \tabularnewline
 & \multicolumn{1}{l|}{} &  & \tabularnewline
\hline 
\multicolumn{2}{c|}{rank} & \multicolumn{2}{c}{perfect matching}\tabularnewline
\hline 
maximum bipartite matching  & \Cref{thm:bipartiteMatchingReduction}  & maximum matching & \Cref{cor:strongReachabilityReduction} \tabularnewline
 & \multicolumn{1}{l}{} &  & \tabularnewline
\hline 
\multicolumn{2}{l|}{maximum matching} & \multicolumn{2}{l}{transitive closure}\tabularnewline
\hline 
counting ST-paths  & \Cref{thm:stPathCountingReduction} & strong connectivity  & \Cref{cor:strongReachabilityReduction} \tabularnewline
\end{tabular}

\caption{\label{fig:reductionOverview}
This table lists all applications and the theorems where these reduction can be found.
}
\end{figure}

==> introtables.tex <==

{\tiny
\begin{tabular}{>{\centering}p{0.15\textwidth}|>{\centering}p{0.08\textwidth}|>{\centering}p{0.07\textwidth}||>{\centering}p{0.08\textwidth}|>{\centering}p{0.08\textwidth}|>{\centering}p{0.15\textwidth}|>{\centering}p{0.1\textwidth}}
\hline 
Variants & Known upper bound & Known lower bound & New upper bound & New lower bound & Corresponding conjectures & References\tabularnewline
\hline 
\hline 
Element update & $O(n^{\OLDfastExponent})$ & \multirow{4}{0.1\textwidth}{$\Omega(n)$} & \elementColor{$O(n^{\fastExponent})$} & \elementColor{$\Omega(n^{\fastExponentLB})$} & \multirow{4}{0.15\textwidth}{\doubleHintedOuMv{} \Cref{con:2hintedOuMv}} & \multirow{4}{0.1\textwidth}{}\tabularnewline
Element query & $O(n^{\OLDfastExponent})$ &  & \elementColor{$O(n^{\fastExponent})$} & \elementColor{$\Omega(n^{\fastExponentLB})$} &  & \tabularnewline
\cline{2-2} 
 & $O(n^{\slowExponent})$ &  &  &  &  & \tabularnewline
 & $O(n^{\slowExponentQuery})$ &  &  &  &  & \tabularnewline
\hline 
Element update & $O(n^{\slowExponent})$ & \multirow{2}{0.1\textwidth}{$\Omega(n)$} & - & \multirow{2}{0.1\textwidth}{\mixedColor{$\Omega(n^{\slowExponent})$}} & \multirow{2}{0.15\textwidth}{\doubleHintedOMv{} \Cref{con:doubleHintedOMv}} & \multirow{2}{0.1\textwidth}{}\tabularnewline
Row query & $O(n^{\slowExponent})$ &  &  &  &  & \tabularnewline
\hline 
Column update & $O(n^{2})$ & \multirow{2}{0.1\textwidth}{$\Omega(n^{\omega-1})$} & \columnColor{$O(n^{\slowExponent})$} & \multirow{2}{0.1\textwidth}{\columnColor{$\Omega(n^{\slowExponent})$}} & \multirow{2}{0.15\textwidth}{\hintedOMv{} \Cref{con:hintedOMv}} & \multirow{2}{0.1\textwidth}{}\tabularnewline
Row query & $O(n)$ &  & \columnColor{$O(n^{\slowExponent})$} &  &  & \tabularnewline
\hline 
\end{tabular}
}

{\tiny
% Preview source code for paragraph 4

\begin{tabular}{>{\centering}p{0.15\textwidth}|>{\centering}p{0.14\textwidth}|>{\centering}p{0.14\textwidth}||>{\centering}p{0.14\textwidth}|>{\centering}p{0.15\textwidth}|c}
\hline 
Variants & Known upper bound & Known upper bound & New upper bound & New upper bound & References\tabularnewline
 & ($O(n)$ look-ahead) & ($O(n^{0.5})$ look-ahead) & ($O(n)$ look-ahead) & ($O(n^{0.5})$ look-ahead) & \tabularnewline
\hline 
\hline 
Dynamic matrix rank &  &  &  &  & \tabularnewline
Type of look-ahead & row and column indices &  & column indices & column indices & \tabularnewline
Element update & $O(n^{\omega-1})$ & missing & $O(n^{\omega-1})$ & $O(n^{\smallLookAhead})$ & \tabularnewline
\hline 
Dynamic matrix inverse &  &  &  &  & \tabularnewline
Type of look-ahead & column indices and values

(row indices for queries) &  & column indices

(row indices for queries) & column indices

(row indices for queries) & \tabularnewline
Column update & $O(n^{\omega-1})$ & missing & $O(n^{\omega-1})$ & $O(n^{\smallLookAhead})$ & \tabularnewline
Row query (for inverse) & $O(n^{\omega-1})$ & missing & $O(n^{\omega-1})$ & $O(n^{\smallLookAhead})$ & \tabularnewline
\hline 
\end{tabular}

}


==> polynomial.tex <==

\section{Polynomial Matrices}
\label{sec:polynomialMatrix}

So far we explained how to maintain the inverse of a matrix over some field, now we extend these results to polynomial matrices. This allows us to get further graph applications such as $k$-cycle detection (\Cref{thm:kCycleReduction}) and all-pairs-shortest-distances (\Cref{thm:shortestDistanceReduction}) and at the end of this section, we are also able to construct a division free dynamic determinant and dynamic adjoint algorithm (see Corollary \ref{cor:ringAdjointDeterminant}) that works on rings instead of fields. The ideas on how to extend our algorithms to the polynomial and division free setting are from \cite{Sankowski05} and \cite{Strassen73}. The proofs for supporting polynomial matrix inversion, division free alogorithms and the all-pairs-shortest-distance reduction are all almost identical to \cite{Sankowski05} by Sankowski, we simply verify that they still apply to our new algorithms. Readers familar with \cite{Sankowski05} can skip ahead to subsection \ref{sub:kCycle}, where the reduction for $k$-cycles is proven.

We will start this section with the results for polynomial matrices and the division free algorithms. In the later subsections \ref{sub:APSD} and \ref{sub:kCycle} we will prove the graph theoretic applications of the polynomial matrix algorithms.

The first main result of this section will be the following Theorem:
\begin{theorem}\label{cor:polyElementUpdate}
Let $\mathbf{R}$ be some ring and $m \in \mathbb{N}$. Let $A$ be a $n \times n$ matrix over $\mathbf{R}[X]/\langle X^{m} \rangle$ (the ring of polynomials modulo $X^m$).

Then all our dynamic matrix inverse algorithms (\Cref{thm:columnUpdate}, \Cref{thm:elementUpdate}, \Cref{thm:inverseSubmatrix}, \Cref{thm:elementLookAhead} and \Cref{thm:columnLookAhead}) can be extended to maintain the inverse of $\I-X \cdot A$ with updates to $A$.

The number of ring operations over $\mathbf{R}$ for pre-processing, updates and queries increase by a factor of $\tilde{O}(m)$.\footnote{Here $\tilde{O}$ hides polylog factors.}
\end{theorem}

\begin{proof}

Note that we want to maintain the inverse of a matrix $\I-X \cdot A$ in $(\mathbf{R}[X]/\langle X^{m} \rangle)^{n \times n}$, i.e. a polynomial matrix modulo $X^m$. The inverse of such a matrix is given by $(\I - X \cdot A)^{-1} = \sum_{k=0}^{m-1} X^k A^k$. To see this, simply multiply both sides with $\I - X \cdot A$, which yields $(\I-X \cdot A)\sum_{k=0}^{m-1} X^k A^k = \sum_{k=0}^{m-1} X^k A^k - \sum_{k=1}^{m} X^k A^k = \I \mod X^m$.

All field operations performed in our algorithms are expressed as matrix operations (i.e. matrix product or matrix inversion), so to prove that our algorithms work over the ring $\mathbf{R}[X]/\langle X^{m} \rangle$ instead of some field, we only have to check that all these matrix operations are well-defined. For matrix multiplication this is obviously true, additionally the number of required operations increases by only a factor of $\tilde{O}(m)$ when using polynomials instead of field elements, because the product of two polynomials of degree at most $m$ can be computed in $O(m \log m)$ using fast fourier transformations.

For the matrix inverse, we have to argue a bit more. We do not have any division operation available for polynomials, so beforehand it is not quite clear if the matrix inverses, which our algorithms try to compute, exist.

We claim that if our algorithms maintain the inverse of $\I - X \cdot A \mod X^m$ and allow the updates to only be performed to $A$, then all matrices that our algorithms have to invert are of the form $\I - X \cdot M$ as well, where $M$ is some polynomial matrix over $\mathbf{R}[X]/\langle X^{m} \rangle$. Matrices of this form can be inverted since $(\I - X \cdot M)^{-1} = \sum_{k=0}^{m-1} M^k \mod X^m$. Checking that all matrices, which our algorithms try to invert, are of this form is done in the appendix \ref{app:polynomialMatrix}.

Next, we have to check how we can efficiently compute the inverse of some matrix $\I - X \cdot M$. We have $(\I - X \cdot M)^{-1} = \sum_{k=0}^{m-1} M^k = \prod_{k=1}^{\log m} (\I + M^{2^k}) \mod X^m$, so the inverse can be computed in $O(\log m)$ matrix multiplications. Given that all computations are performed modulo $X^m$ the degrees are always bounded by $X^{m-1}$, so each matrix product becomes slower by only $O(m \log m)$ operations. Hence in total we can invert any polynomial $n \times n$ matrix mod $X^m$ in $\tilde{O}(m n^\omega)$ time, so the matrix inversion becomes slower by a factor of $\tilde{O}(m)$.

By performing all matrix inversions in our algorithms this way, we can extend the algorithms to the polynomial setting, where we have to maintain the inverse of a polynomial matrix $\I - X \cdot A \mod X^m$, when the updates are performed to matrix $A$. The number of arithmetic operations performed by the algorithms increase by a factor of $\tilde{O}(m)$.


\end{proof}

The reduction from dynamic matrix inverse to dynamic determinant from Theorem \ref{thm:inverseDeterminantEquivalence} via the identity $\det(M + u v^\top) = \det(M)(1 + v^\top M^{-1} u)$ still holds in the polynomial setting for $M = \I - X \cdot A$, so by maintaining the inverse modulo $X^m$, we can also maintain the determinant modulo $X^m$. The same is also true for the reduction from adjoint to inverse (\Cref{cor:inverseAdjointEquivalence}) via the identity $adj(M) = \det(M)M^{-1}$.

\begin{corollary}\label{cor:polyElementUpdateDeterminant}
Let $\mathbf{R}$ be some ring and $m \in \mathbb{N}$. Let $A$ be a $n \times n$ matrix over $\mathbf{R}[X]/\langle X^{m} \rangle$ (the ring of polynomials modulo $X^m$).

Then our dynamic matrix inverse algorithms (Theorem \ref{thm:columnUpdate}, Theorem \ref{thm:elementUpdate}, \Cref{thm:elementLookAhead} and \Cref{thm:columnLookAhead}) can be used to maintain the determinant (or adjoint) of $\I-X \cdot A$, supporting updates to $A$.

The number of ring operations over $\mathbf{R}$ for pre-processing, updates and queries increase by a factor of $\tilde{O}(m)$.
\end{corollary}


\paragraph{Division free dynamic adjoint and determinant algorithms} In \cite{Sankowski05} Sankowski explained how to extend the techniques from \cite{Strassen73} to dynamically maintain the adjoint and the determinant without using divisions, resulting in an algorithm that can be used on rings instead of fields.

For this observe that $\det(\I-X\cdot(\I-A)) = \det(A)$ for $X=1$, so we only have to maintain the determinant of the polynomial matrix $\I-X\cdot(\I-A)$ and evaluate it for $X=1$ after every update. The matrix $\I-X\cdot(\I-A)$ is of the form $\I-X\cdot A'$, so we can use the algorithm from \Cref{cor:polyElementUpdate} to maintain the determinant of the polynomial matrix modulo some $X^m$. Since the polynomial $\det(\I-X\cdot(\I-A))$ is of degree at most $n$, we choose to run our algorithm modulo $X^{n+1}$, so the runtime of our matrix inverse/determinant algorithms increase by a factor of $\tilde{O}(m) = \tilde{O}(n)$.

Similarly we have $adj(A) = adj(\I-X\cdot(\I-A))$ for $X=1$ and $adj(\I-X\cdot(\I-A)) = \det(\I-X\cdot(\I-A)) \cdot (I-X\cdot(\I-A))^{-1} \mod X^{n}$, so we can also maintain the adjoint of $A$ by maintaining the inverse and determinant of the polynomial matrix $\I-X\cdot(\I-A)$.

\begin{corollary}\label{cor:ringAdjointDeterminant}
Let $\mathbf{R}$ be a ring, then the algorithms from Theorem \ref{thm:columnUpdate}, Theorem \ref{thm:elementUpdate}, \Cref{thm:elementLookAhead} and \Cref{thm:columnLookAhead} can be extended to maintain the determinant and adjoint of a matrix $A \in \mathbf{R}^{n \times n}$. The required ring operations for pre-processing, updates and queries increase by a factor of $\tilde{O}(n)$. 
\end{corollary}


\subsection{Polynomial Matrices for All-Pairs-Shortest-Distances}
\label{sub:APSD}

In this subsection we will prove the reduction for all-pairs-shortest-distance (Theorem \ref{thm:APSPreduction}). The following reduction is almost identical to the one used in \cite{Sankowski05} by Sankowski, the only difference is that Sankowski used the adjoint of a polynomial matrix, while we use the inverse.

We will start with the outline of how we can obtain the distances in a graph from the polynomial matrix inverse: Let $m \in \mathbb{N}$ and let $A$ be the adjacency matrix of a graph, then the inverse of $\I - X \cdot A$ modulo $X^m$ is given by $\sum_{k=0}^{m-1} X^k A^k$. This means the entry $(\I - X \cdot A)^{-1}_{i,j}$ is a polynomial where the coefficient of the $k$th monomial (for $k < m$) is exactly the number of walks of length $k$ from $i$ to $j$. So by looking for the smallest non-zero monomial, the inverse encodes the shortest distances upto length $m-1$ in the graph. This can be extended to weighted graphs with integer edge weights $c_{i,j}$, by setting $A_{i,j} = X^{c_{i,j}-1}$. One issue with this type of reduction is, that the coefficients of $A^k$ could become rather large, i.e. bit-length $\Omega(n)$. We will fix the issue later in the proof of Theorem \ref{thm:APSPreduction}.

When considering this graph application, the parameter $m$ bounds the maximum distance we can compute. This is useful because it allows for runtime improvements using a hitting set argument for $m << n$.

The following reduction exploits an observation by Ullman and Yannakakis \cite{UllmanY91}, which can be informally described as follows: If some path happens to be long, then it must visit many nodes. Thus by sampling some random nodes $H \subset V$, Ullman and Yannakakis proved that a long path must visit nodes from $H$ w.h.p. and any path from $i$ to $j$ can thus be decomposed (w.h.p) into segments $i \to h_1, h_1 \to h_2, ... h_k \to j$ of shorter length, where $h_1,...,h_k \in H$.

\begin{theorem}\label{thm:APSPreduction}
Let $0 \le \mu \le 1$, $I,J \subset [n]$ and let $A \in \mathbf{F}^{n \times n}$ be a polynomial matrix over some finite field $\mathbf{F}$.

There exists a $k = O(n^{1-\mu})$ such that for a uniformly at random chosen $H \subset [n]$, $|H| = k$ the following is true:

Assume there exists a dynamic algorithm $\mathcal{I}$ for maintaining the inverse $(I-X\cdot A)^{-1} \mod X^{n^\mu}$, where the pre-processing requires $O(p(n^\mu,n))$ operations, element updates to $A$ require $O(u(n^\mu,n))$ operations. Further assume element queries to $(\I - X \cdot A)^{-1} \mod X^{n^\mu}$ and queries to obtain any partial row $(\I - X \cdot A)^{-1}_{i,H}$ for any row index $i$, both require $O(q(n^\mu,n))$ operations, additionally $\mathcal{I}$ maintains the submatrix $((I-X \cdot A)^{-1})_{H,H} \mod X^{n^\mu}$ explicitly.

Then there exists a randomized dynamic algorithm for the (unweighted, directed) all pairs shortest distance problem with pre-processing time $\tilde{O}(p(n^\mu,n)+n^{3-3\mu})$, edge update time $\tilde{O}(u(n^\mu,n)+n^{3-3\mu})$ and pair query time $\tilde{O}(q(n^\mu,n)+n^{2-2\mu})$.
\end{theorem}

\begin{proof}
Assume for now $\mathbf{F} = \mathbb{Z}$, even though it is not a field and let $A$ be the adjacency matrix of the graph. We already know for $m = n^\mu$ that $(\I-X \cdot A)^{-1} = \sum_{k=0}^{m} X^k A^k \mod X^m$, which means the smallest monomial at entry $(i,j)$ will give use the distance between nodes $i$ and $j$, if the shortest distance is less than $m$. The coefficient of this monomial is the number of such shortest paths, so the coefficient could require a bit-length of $\Omega(n)$, which would result in a increased complexity. We can fix the following way: Let $\mathbf{F} = \mathbb{Z}_p$ for a large prime $p \sim n^c$ for some large enough constant $c$. Each non-zero entry of $A$ is an independently and uniformly at random chosen element from $\mathbb{Z}_p$, then $A^k_{i,j}$ is non-zero w.h.p, if and only if there exists a walk from $i$ to $j$ of length $k$ (see Schwatz-Zippel Lemma \ref{lem:schwartzZippel}). Hence we can maintain w.h.p all the shortest distances with length less than $m$ by maintaining $(\I-X\cdot A)^{-1} \mod X^{m}$. For $m$ large enough but $m << n$, this is already enough to compute the shortest distances w.h.p using the following property due to Ullman and Yannakakis \cite[Lemma 2.2]{UllmanY91}:\smallskip

\emph{If we choose $H \subset V$ to be a uniformly at random chosen subset of the vertices, then the probability that a given (acyclic) path has a sequence of more than $(cn \log n)/|H|$ vertices, none of which are in $H$, is, for sufficiently large $n$, bounded from below by $2^{1-\alpha c}$ for some positive $\alpha$.}\smallskip

So for $m = n^\mu$ and $|H| = cn/m \log n = \tilde{O}(n^{1-\mu})$ the shortest paths will use w.h.p at most $m$ nodes not from $H$ in sequence. This means a shortest path from $i$ to $j$ with length larger than $m$ can be decomposed into segments $i \to h_1, h_1 \to h_2, ... h_k \to j$.

Let $D_{i,j}$ be the distance matrix obtained from the smallest monomials of $A^{-1}$. Now consider a new graph with vertices $H$, where an edge $(i,j)$ has weight $D_{i,j}$ (if an entry $(i,j)$ of $(A^{-1})_{H,H}$ is 0, then the edge $(i,j)$ does not exists in this new graph).
We can compute the shortest distances $(B_{i,j})_{i,j\in H}$ in that new graph in $\tilde{O}(n^{3(1-\mu)})$ time using some all-pairs-shortest-path algorithm.

Via \cite{UllmanY91} we now know, that we can get (w.h.p) the shortest distance between any $i$ and $j$ via $\min \{D_{i,j}, \min_{p,q \in H} D_{i,p} + B_{p,q} + D_{q,j}\}$. Thus for every update, we simply compute $B$ from $D_{H,H}$, which increases the update time by $\tilde{O}(n^{3(1-\mu)})$. When we query the distance for some pair $(i,j)$ we have to query the partial row $(\I-A \cdot X)^{-1}_{i,H}$, partial column $(\I-A \cdot X)^{-1}_{H,j}$ and the element $(\I-A \cdot X)^{-1}_{i,j}$ and then compare the distances in $\tilde{O}(n^{2(1-\mu)})$ time. The partial column $(\I-A \cdot X)^{-1}_{H,j}$ can be queried by maintaining $(\I-A \cdot X)^{\top -1}$ in parallel and querying $(\I-A \cdot X)^{\top -1}_{j,H}$.

Hence update and query time become $\tilde{O}(u(n^\mu,n)+n^{3-3\mu})$ and $\tilde{O}(q(n^\mu,n)+n^{2-2\mu})$ respectively.

\end{proof}

\begin{proof}[Proof of \Cref{thm:shortestDistanceReduction}]
By using the algorithm from \Cref{thm:inverseSubmatrix}, we can maintain a submatrix $(A^{-1})_{H,H}$ for some $H \subset [n]$ of the inverse explicitly, if we can query partial rows $(A^{-1})_{i,H}$ for any $i \in [n]$. \Cref{thm:shortestDistanceReduction} is now obtained by applying \Cref{thm:APSPreduction}.
\end{proof}

\begin{corollary}\label{cor:APSP}
For any $0 \le \mu \le 1$, $0 \le \varepsilon_1 \le \varepsilon_2 \le 1$ there exists a dynamic all-pairs-shortest-distance algorithm, that maintains the distance in a directed $n$ node graph, supporting edge updates in $\tilde{O}(n^{\mu}[n^{\varepsilon_1+\varepsilon_2}+n^{\omega(1,\varepsilon_1,\varepsilon_2)-\varepsilon_1}+n^{\omega(1,1,\varepsilon_2)-\varepsilon_2}+n^{\varepsilon_2+1-\mu}+n^{2-2\mu}+n^{3-3\mu}])$ time and queries in $\tilde{O}(n^{\mu}[n^{\varepsilon_1+\varepsilon_2}+n^{\varepsilon_2+1-\mu}+n^{2-2\mu}])$ time. The pre-processing requires $\tilde{O}(n^\mu n^\omega+n^{3-3\mu})$ time.

For current values of $\omega$ this implies an update and query time of $O(n^{1.814})$ for $\varepsilon_1 \approx 0.54, \varepsilon_2 \approx 0.814, \mu \approx 0.395$.
\end{corollary}

The update complexity of \Cref{cor:APSP} stems from:
\begin{align*}
\tilde{O}(n^{\mu}[
\underbrace{
n^{\varepsilon_1+\varepsilon_2}
+n^{\omega(1,\varepsilon_1,\varepsilon_2)-\varepsilon_1}
+n^{\omega(1,1,\varepsilon_2)-\varepsilon_2}
}_{\text{\Cref{thm:elementUpdate}}}
+\underbrace{n^{\varepsilon_2+1-\mu}+n^{2-2\mu}}_{\text{\Cref{cor:elementUpdateSubmatrix}}}
+\underbrace{n^{3-3\mu}}_{\text{\Cref{thm:APSPreduction}}}
])
\end{align*}

While the query complexity is a slower than in \cite{Sankowski05} (see \Cref{tbl:applications}), our update time is faster, which allows for a better runtime in applications with few queries, such as $st$-distance.

\subsection{Polynomial Matrices for $k$-Cycle Detection}
\label{sub:kCycle}

In this subsection we will prove the reduction for $k$-cycle detection (Theorem \ref{thm:kCycleReduction}).
The reduction is based on the observation that the determinant of an adjacency matrix encodes information about the cycles in the graph.

\begin{proof}[Proof of Theorem \ref{thm:kCycleReduction}]
First, let us repeat the theorem:

\emph{Let $\mathcal{D}$ be a dynamic determinant algorithm, that maintains the determinant of $(\I-X \cdot A)^{-1} \in (\mathbf{R}[X]/\langle X^k \rangle)^{n \times n}$ with pre-processing in $O(p(k,n))$ operations (over $\mathbf{R}$) and element updates to $A$ in $O(u(k,n))$ operations (over $\mathbf{R}$).}

\emph{There exists some function $f(k)$, such that there is a dynamic $k$-cycle algorithm $\mathcal{C}$, which detects if a $n$ node graph contains a node disjoint cycle of length $k$, with pre-processing time $O(f(k) \cdot p(k,n))$ and edge update time $O(f(k) \cdot (u(k,n)))$.}\smallskip


The high-level idea of the reduction is to use color coding on the graph and to then detect a cycle in the color coded graph.

Given a graph, we assign each node a independent and uniformly at random chosen color from $\{1,...,k\}$. Then we will only keep those edges that go from nodes of color $i$ to $i+1$ or from color $k$ to color $1$. If there exists a $k$ cycle in the original graph, then with a small but positive probability that depends only on $k$, the cycle still exists in the color coded graph. However, if no $k$-cycle exists in the original graph, then the color coded cycle will also have no $k$-cycle.

Now if we would simply use a cycle detection algorithm (e.g. via Theorem \ref{thm:cycleDetectionReduction}), we might get a false positive by detecting a cycle of length $s\cdot k$ for some $s > 1$. So we have to make sure that our cycle detection algorithm can only detect cycles of length upto $k$. This is where the polynomial matrix comes into play.

The determinant of the matrix $\I - X \cdot A$, where $A$ is the adjacency matrix of the color coded graph, encodes information about the cycles. We have $\det(\I-X\cdot A) = \sum_\sigma \text{sign}(\sigma) \prod_{i=1}^n (\I-X\cdot A)_{i,\sigma(i)}$, where $\prod_{i=1}^n (\I-X\cdot A)_{i,\sigma(i)}$ is non-zero if and only if the cycle decomposition of $\sigma$ represents valid cycles in the graph represented by adjacency matrix $A$. Note that the degree of $\prod_{i=1}^n (\I-X\cdot A)_{i,\sigma(i)}$ is exactly the number of used edges, and since the color coded graph has no cycles of length less than $k$, the degree of $\prod_{i=1}^n A_{i,\sigma(i)}$ is $k$ if and only if the color coded graph has a $k$ cycle.
The only issue now is that maybe some terms cancel because of the sum and $\text{sign}(\sigma)$. However, using Schwartz-Zippel Lemma \ref{lem:schwartzZippel}, we can prove that if we set the entries of $A$ to be random values over some field $\mathbb{Z}_{p}$ where $p \sim n^c$ for some large enough constant $c$, then w.h.p. the $k$th monomial of $det(\I-X \cdot A)$ will be nonzero if and only if there exists no $k$-cycle in the color coded graph.

Now we simply maintain some exponential number $f(k)$ of independently color coded graphs to detect a $k$-cycle w.h.p.

\end{proof}


